Reinforcement Learning in a Physics-Inspired Semi-Markov Environment

Reinforcement learning (RL) has been demonstrated to have great potential in many applications of scientific discovery and design. Recent work includes, for example, the design of new structures and compositions of molecules for therapeutic drugs. Much of the existing work related to the application of RL to scientific domains, however, assumes that the available state representation obeys the Markov property. For reasons associated with time, cost, sensor accuracy, and gaps in scientific knowledge, many scientific design and discovery problems do not satisfy the Markov property. Thus, something other than a Markov decision process (MDP) should be used to plan / find the optimal policy. In this paper, we present a physics-inspired semi-Markov RL environment, namely the phase change environment. In addition, we evaluate the performance of value-based RL algorithms for both MDPs and partially observable MDPs (POMDPs) on the proposed environment. Our results demonstrate deep recurrent Q-networks (DRQN) significantly outperform deep Q-networks (DQN), and that DRQNs benefit from training with hindsight experience replay. Implications for the use of semi-Markovian RL and POMDPs for scientific laboratories are also discussed.

==> library.tex <==
@article{aag_rl_2019,
  title={Exploring the chemical space without bias: data-free molecule generation with {DQN} and {SELFIES}},
  journal={NeurIPS ML4PS Workshop},
  year={2019},
  author={Gaudin, Th{\'e}ophile and Nigam, AkshatKumar and Aspuru-Guzik, Alan}
}

@article{hein_robot_2019,
author = {Daponte, Jordan A. and Guo, Yuejun and Ruck, Rebecca T. and Hein, Jason E.},
title = {Using an automated monitoring platform for investigations of biphasic reactions},
journal = {ACS Catalysis},
volume = {9},
number = {12},
pages = {11484-11491},
year = {2019}
}

@Article{cooper_robots_2018,
author={Greenaway, R. L. and others},
title={High-throughput discovery of organic cages and catenanes using computational screening fused with robotic synthesis},
journal={Nature Communications},
year={2018},
volume={9},
number={1},
pages={2849},
issn={2041-1723}
}
%author={Greenaway, R. L. and Santolini, V. and Bennison, M. J. and Alston, B. M. and Pugh, C. J. and Little, M. A. and Miklitz, M. and Eden-Rump, E. G. B. and Clowes, R. and Shakil, A. and Cuthbertson, H. J. and Armstrong, H. and Briggs, M. E. and Jelfs, K. E. and Cooper, A. I.},


@article{cronin_chemputer_2018,
	author = {Steiner, Sebastian and others},
	title = {Organic synthesis in a modular robotic system driven by a chemical programming language},
	volume = {363},
	number = {6423},
	elocation-id = {eaav2211},
	year = {2019},
	publisher = {American Association for the Advancement of Science},
	journal = {Science}
}
%author = {Steiner, Sebastian and Wolf, Jakob and Glatzel, Stefan and Andreou, Anna and Granda, Jaros{\l}aw M. and Keenan, Graham and Hinkley, Trevor and Aragon-Camarasa, Gerardo and Kitson, Philip J. and Angelone, Davide and Cronin, Leroy},


@BOOK{Decadal_2019,
  author    = "National Academies of Sciences, Engineering, and Medicine",
  title     = "Frontiers of Materials Research: A Decadal Survey",
  abstract  = "Modern materials science builds on knowledge from physics, chemistry, biology, mathematics, computer and data science, and engineering sciences to enable us to understand, control, and expand the material world. Although it is anchored in inquiry-based fundamental science, materials research is strongly focused on discovering and producing reliable and economically viable materials, from super alloys to polymer composites, that are used in a vast array of products essential to today\u2019s societies and economies.\n\nFrontiers of Materials Research: A Decadal Survey is aimed at documenting the status and promising future directions of materials research in the United States in the context of similar efforts worldwide. This third decadal survey in materials research reviews the progress and achievements in materials research and changes in the materials research landscape over the last decade; research opportunities for investment for the period 2020-2030; impacts that materials research has had and is expected to have on emerging technologies, national needs, and science; and challenges the enterprise may face over the next decade.",
  year      = 2019,
  publisher = "The National Academies Press",
  address   = "Washington, DC"
}

@misc{openAIGym2016,
  Author = {Greg Brockman and others},
  Title = {OpenAI Gym},
  Year = {2016},
  Eprint = {arXiv:1606.01540},
}
%  Author = {Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},

@inproceedings{andrychowicz2017hindsight,
  title={Hindsight experience replay},
  author={Andrychowicz, Marcin and others},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5048--5058},
  year={2017}
}
%author={Andrychowicz, Marcin and Wolski, Filip and Ray, Alex and Schneider, Jonas and Fong, Rachel and Welinder, Peter and McGrew, Bob and Tobin, Josh and Abbeel, OpenAI Pieter and Zaremba, Wojciech},

@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and others},
  journal={Nature},
  volume={518},
  number={7540},
  pages={529},
  year={2015},
  publisher={Nature Publishing Group}
}
%author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},

@inproceedings{hausknecht2015deep,
  title={Deep recurrent {Q}-learning for partially observable {MDP}s},
  author={Hausknecht, Matthew and Stone, Peter},
  booktitle={2015 AAAI Fall Symposium Series},
  year={2015}
}
@inproceedings{mnih2013playing,
  title={Playing Atari with deep reinforcement learning},
  author={Mnih, Volodymyr and others},
  booktitle={NeurIPS: Deep Learning Workshop},
  year={2013}
}
%author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin}


@article{silver2016mastering,
  title={Mastering the game of {Go} with deep neural networks and tree search},
  author={Silver, David and others},
  journal={Nature},
  volume={529},
  number={7587},
  pages={484},
  year={2016},
  publisher={Nature Publishing Group}
}
%  author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
@inproceedings{gu2017deep,

  title={Deep reinforcement learning for robotic manipulation with asynchronous off-policy updates},
  author={Gu, Shixiang and Holly, Ethan and Lillicrap, Timothy and Levine, Sergey},
  booktitle={2017 IEEE international conference on robotics and automation (ICRA)},
  pages={3389--3396},
  year={2017},
  organization={IEEE}
}
@article{zhou2019optimization,
  title={Optimization of molecules via deep reinforcement learning},
  author={Zhou, Zhenpeng and Kearnes, Steven and Li, Li and Zare, Richard N and Riley, Patrick},
  journal={Scientific reports},
  volume={9},
  number={1},
  pages={1--10},
  year={2019},
  publisher={Nature Publishing Group}
}
@article{popova2018deep,
  title={Deep reinforcement learning for de novo drug design},
  author={Popova, Mariya and Isayev, Olexandr and Tropsha, Alexander},
  journal={Science advances},
  volume={4},
  number={7},
  pages={eaap7885},
  year={2018},
  publisher={American Association for the Advancement of Science}
}
@article{zhou2017optimizing,
  title={Optimizing chemical reactions with deep reinforcement learning},
  author={Zhou, Zhenpeng and Li, Xiaocheng and Zare, Richard N},
  journal={ACS central science},
  volume={3},
  number={12},
  pages={1337--1344},
  year={2017},
  publisher={ACS Publications}
}

@article{roch2018chemos,
  title={ChemOS: Orchestrating autonomous experimentation},
  author={Roch, Lo{\"\i}c M and others},
  journal={Science Robotics},
  volume={3},
  number={19},
  pages={eaat5559},
  year={2018},
  publisher={Science Robotics}
}
%  author={Roch, Lo{\"\i}c M and H{\"a}se, Florian and Kreisbeck, Christoph and Tamayo-Mendoza, Teresa and Yunker, Lars PE and Hein, Jason E and Aspuru-Guzik, Al{\'a}n},

@article{macleod2019self,
  title={Self-driving laboratory for accelerated discovery of thin-film materials},
  author={MacLeod, Benjamin P and others},
  journal={arXiv preprint arXiv:1906.05398},
  year={2019}
}
%author={MacLeod, Benjamin P and Parlane, Fraser GL and Morrissey, Thomas D and H{\"a}se, Florian and Roch, Lo{\"\i}c M and Dettelbach, Kevan E and Moreira, Raphaell and Yunker, Lars PE and Rooney, Michael B and Deeth, Joseph R and others},

@article{whitelam2019learning,
  title={Learning to grow: control of materials self-assembly using evolutionary reinforcement learning},
  author={Whitelam, Stephen and Tamblyn, Isaac},
  journal={arXiv preprint arXiv:1912.08333},
  year={2019}
}

@article{nautrup2019optimizing,
  title={Optimizing quantum error correction codes with reinforcement learning},
  author={Nautrup, Hendrik Poulsen and Delfosse, Nicolas and Dunjko, Vedran and Briegel, Hans J and Friis, Nicolai},
  journal={Quantum},
  volume={3},
  pages={215},
  year={2019},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}
@article{andreasson2019quantum,
  title={Quantum error correction for the toric code using deep reinforcement learning},
  author={Andreasson, Philip and Johansson, Joel and Liljestrand, Simon and Granath, Mats},
  journal={Quantum},
  volume={3},
  pages={183},
  year={2019},
  publisher={Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften}
}
@article{fosel2018reinforcement,
  title={Reinforcement learning with neural networks for quantum feedback},
  author={F{\"o}sel, Thomas and Tighineanu, Petru and Weiss, Talitha and Marquardt, Florian},
  journal={Physical Review X},
  volume={8},
  number={3},
  pages={031084},
  year={2018},
  publisher={APS}
}
@article{jiang2018joint,
  title={Joint activity detection and channel estimation for IoT networks: phase transition and computation-estimation tradeoff},
  author={Jiang, Tao and Shi, Yuanming and Zhang, Jun and Letaief, Khaled B},
  journal={IEEE Internet of Things Journal},
  year={2018},
  publisher={IEEE}
}
@phdthesis{watkins1989learning,
  title={Learning from delayed rewards},
  author={Watkins, Christopher John Cornish Hellaby},
  year={1989},
  school={King's College, Cambridge}
}
@inproceedings{schaul2015universal,
  title={Universal value function approximators},
  author={Schaul, Tom and Horgan, Daniel and Gregor, Karol and Silver, David},
  booktitle={International Conference on Machine Learning},
  pages={1312--1320},
  year={2015}
}
@incollection{sutton1990integrated,
  title={Integrated architectures for learning, planning, and reacting based on approximating dynamic programming},
  author={Sutton, Richard S},
  booktitle={Machine Learning Proceedings 1990},
  pages={216--224},
  year={1990},
  publisher={Elsevier}
}

